Towards Domain Independence in CNN-based Acoustic Localization using Deep Cross Correlations

Time delay estimation is essential in Acoustic Source Localization (ASL) systems. One of the most used techniques for this purpose is the Generalized Cross Correlation (GCC) between a pair of signals and its use in Steered Response Power (SRP) techniques, which estimate the acoustic power at a specific location. Nowadays, Deep Learning strategies may outperform these methods. However, they are generally dependent on the geometric and sensor configuration conditions that are available during the training phases, thus having limited generalization capabilities when facing new environments if no re-training nor adaptation is applied. In this work, we propose a method based on an encoder-decoder CNN architecture capable of outperforming the well known SRP-PHAT algorithm, and also other Deep Learning strategies when working in mismatched training-testing conditions without requiring a model re-training. Our proposal aims to estimate a smoothed version of the correlation signals, that is then used to generate a refined acoustic power map, which leads to better performance on the ASL task. Our experimental evaluation uses three publicly available realistic datasets and provides a comparison with the SRP-PHAT algorithm and other recent proposals based on Deep Learning.

==> figure-RoomLayout.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.30\textwidth}
    \includegraphics[width=\textwidth]{roomlayout2}
    \caption{}
    \label{fig:RoomLayout}
  \end{subfigure}%
  \qquad \qquad %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
  % (or a blank line to force the subfigure onto a new line)
  \begin{subfigure}[b]{0.425\textwidth}
    \includegraphics[width=\textwidth]{idiap-seq45-cam2.jpg}
    \caption{}
    \label{fig:RoomPicture}
  \end{subfigure}
  \caption{IDIAP Smart Meeting Room for AV16.3 recordings.
    (\protect\subref{fig:RoomLayout}) Room layout showing the centered
    table, and the microphones arranged in two circular arrays.
    (\protect\subref{fig:RoomPicture}) Sample of recorded video frame
    showing the arrays area. \vspace{-0.3cm}}
  \label{fig:LIdiapRoom}
\end{figure}


==> table-cav3d-av163-upc-itc-high.tex <==

\begin{table}[htb]
	\centering
  \resizebox{\columnwidth}{!}{
    % \footnotesize
    \begin{tabular}{| c | c | c || c | c | c |}
      \hline
      \textbf{\textit{CAV3D}} & \textbf{\#} & \textbf{Feats} & \textbf{\textit{AV16.3}} & \textbf{\#}  & \textbf{Feats} \\
      \hline \hline
      \texttt{Cseq06} & 393 & $M$     & \texttt{Aseq01}  & 1328 & $S+3$ \\
      \hline
      \texttt{Cseq07} & 374 & $M$     & \texttt{Aseq0f2} & 1441 & $S+3$ \\
      \hline
      \texttt{Cseq08} & 412 & $M$     & \texttt{Aseq03}  & 1552 & $S+3$ \\
      \hline
      \texttt{Cseq09} & 367 & $M+1$   & \texttt{Aseq11}  &  297 & $M+3$ \\
      \hline
      \texttt{Cseq10} & 245 & $M+1$   & \texttt{Aseq15}  &  284 & $M+3$ \\
      \hline
      \texttt{Cseq11} & 709 & $M+1+2$ & ---              &  --- &   --- \\
      \hline
      \texttt{Cseq12} & 725 & $M+1+2$ &             ---  &  --- &   --- \\
      \hline
      \texttt{Cseq13} & 684 & $M+3$   &             ---  &  --- &   --- \\
      \hline
      \texttt{Cseq20} & 422 & $M$     &             ---  &  --- &   --- \\
      \hline
      \texttt{Cseq21} & 476 & $M+2$   &             ---  &  --- &   --- \\
      \hline
      \hline
      \textbf{\textit{UPC}} & \textbf{\#}  & \textbf{Feats} & \textbf{\textit{ITC}} & \textbf{\#}  & \textbf{Feats}\\
      \hline
      \texttt{Useq01} & 3869 & $S+3$ & ---              &  --- &   --- \\
      \hline                                  
      \texttt{Useq02} & 4455 & $S+3$ & ---              &  --- &   --- \\
      \hline                          
      \texttt{Useq03} & 3794 & $S+3$ & ---              &  --- &   --- \\
      \hline                  
      \texttt{Useq04} & 3780 & $S+3$ & ---              &  --- &   --- \\
      \hline          
      \texttt{Useq05} & 4348 & $S+3$ & ---              &  --- &   --- \\
      \hline  
      \texttt{Useq06} & 3915 & $S+3$ & ---              &  --- &   --- \\
      \hline
      \texttt{Useq07} & 3135 & $S+3$ & ---              &  --- &   --- \\
      \hline
      \texttt{Useq08} & 3734 & $S+3$ & ---              &  --- &   --- \\
      \hline
      ---             &  --- &   --- & ---              &  --- &   --- \\
      \hline
      ---             &  --- &   --- & ---              &  --- &   --- \\
      \hline






    \end{tabular}
  }
	\caption{\textit{CAV3D}, \textit{AV16.3}, \textit{UPC} sequences used to train and test our method. Second and fifth columns are the number of available acoustic frames in the sequence and third and last columns represent the features in the sequence}
	\label{tab:table2}
\end{table}



==> table-cav3d-av163-upc-itc-wide-short.tex <==
\begin{table}[htb]
	\centering
  \resizebox{\columnwidth}{!}{
    % \footnotesize
    \begin{tabular}{| c | c | c || c | c | c || c | c | c || c | c | c |}
      \hline
      \textbf{\textit{CAV3D}} & \textbf{\#} & \textbf{Feats} & \textbf{\textit{AV16.3}} & \textbf{\#}  & \textbf{Feats} & \textbf{\textit{UPC}} & \textbf{\#}  & \textbf{Feats} & \textbf{\textit{ITC}} & \textbf{\#}  & \textbf{Feats}\\
      \hline \hline
      \texttt{C06} & 393 & $M$     & \texttt{A01}  & 1328 & $S+3$ & \texttt{U01} & 3869 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{C07} & 374 & $M$     & \texttt{A0f2} & 1441 & $S+3$ & \texttt{U02} & 4455 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{C08} & 412 & $M$     & \texttt{A03}  & 1552 & $S+3$ & \texttt{U03} & 3794 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{C09} & 367 & $M+1$   & \texttt{A11}  &  297 & $M+3$ & \texttt{U04} & 3780 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{C10} & 245 & $M+1$   & \texttt{A15}  &  284 & $M+3$ & \texttt{U05} & 4348 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{C11} & 709 & $M+1+2$ & ---              &  --- &   --- & \texttt{U06} & 3915 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{C12} & 725 & $M+1+2$ &             ---  &  --- &   --- & \texttt{U07} & 3135 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{C13} & 684 & $M+3$   &             ---  &  --- &   --- & \texttt{U08} & 3734 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{C20} & 422 & $M$     &             ---  &  --- &   --- & ---             &  --- &   --- & ---             &  --- &   --- \\
      \hline
      \texttt{C21} & 476 & $M+2$   &             ---  &  --- &   --- & ---             &  --- &   --- & ---             &  --- &   --- \\
      \hline
    \end{tabular}
  }
	\caption{Details on the \textit{CAV3D}, \textit{AV16.3}, \textit{UPC}
    and \textit{ITC} sequences used to train and test our method. Second and fifth columns are the number of available acoustic frames in the sequence and third and last columns represent the features in the sequence}
	\label{tab:table2}
\end{table}



==> table-cav3d-av163-upc-itc-wide.tex <==
\begin{table}[htb]
	\centering
  \resizebox{\columnwidth}{!}{
    % \footnotesize
    \begin{tabular}{| c | c | c || c | c | c || c | c | c || c | c | c |}
      \hline
      \textbf{\textit{CAV3D}} & \textbf{\#} & \textbf{Feats} & \textbf{\textit{AV16.3}} & \textbf{\#}  & \textbf{Feats} & \textbf{\textit{UPC}} & \textbf{\#}  & \textbf{Feats} & \textbf{\textit{ITC}} & \textbf{\#}  & \textbf{Feats}\\
      \hline \hline
      \texttt{Cseq06} & 393 & $M$     & \texttt{Aseq01}  & 1328 & $S+3$ & \texttt{Useq01} & 3869 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{Cseq07} & 374 & $M$     & \texttt{Aseq0f2} & 1441 & $S+3$ & \texttt{Useq02} & 4455 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{Cseq08} & 412 & $M$     & \texttt{Aseq03}  & 1552 & $S+3$ & \texttt{Useq03} & 3794 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{Cseq09} & 367 & $M+1$   & \texttt{Aseq11}  &  297 & $M+3$ & \texttt{Useq04} & 3780 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{Cseq10} & 245 & $M+1$   & \texttt{Aseq15}  &  284 & $M+3$ & \texttt{Useq05} & 4348 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{Cseq11} & 709 & $M+1+2$ & ---              &  --- &   --- & \texttt{Useq06} & 3915 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{Cseq12} & 725 & $M+1+2$ &             ---  &  --- &   --- & \texttt{Useq07} & 3135 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{Cseq13} & 684 & $M+3$   &             ---  &  --- &   --- & \texttt{Useq08} & 3734 & $S+3$ & ---             &  --- &   --- \\
      \hline
      \texttt{Cseq20} & 422 & $M$     &             ---  &  --- &   --- & ---             &  --- &   --- & ---             &  --- &   --- \\
      \hline
      \texttt{Cseq21} & 476 & $M+2$   &             ---  &  --- &   --- & ---             &  --- &   --- & ---             &  --- &   --- \\
      \hline
    \end{tabular}
  }
	\caption{\textit{CAV3D}, \textit{AV16.3}, \textit{UPC} sequences used to train and test our method. Second and fifth columns are the number of available acoustic frames in the sequence and third and last columns represent the features in the sequence}
	\label{tab:table2}
\end{table}


